A Model for Variation- and Fault-Tolerant Digital Logic using Self-Assembled Nanowire Architectures

Reconfiguration has been used for both defect- and fault-tolerant nanoscale architectures with regular structure. Recent advances in self-assembled nanowires have opened doors to a new class of electronic devices with irregular structure. For such devices, reservoir computing has been shown to be a viable approach to implement computation. This approach exploits the dynamical properties of a system rather than specifics of its structure. Here, we extend a model of reservoir computing, called the echo state network, to reflect more realistic aspects of self-assembled nanowire networks. As a proof of concept, we use echo state networks to implement basic building blocks of digital computing: AND, OR, and XOR gates, and 2-bit adder and multiplier circuits. We show that the system can operate perfectly in the presence of variations five orders of magnitude higher than ITRS's 2005 target, $\bm{6\%}$, and achieves success rates $\bm{6}$ times higher than related approaches at half the cost. We also describe an adaptive algorithm that can detect faults in the system and reconfigure it to resume perfect operational condition.

==> takeout.tex <==
 In our experiments we showed that ESN is robust to high level of variations, i.e., $\approx 100,000\%$ of the defined characteristics, which is 5 orders of magnitude higher than the target variation and what has been reported by ITRS and the industry\cite{4447311}. To see this we have to mention that the magnitude of average weight in our system is $\mu\approx 0.0001$ and we used variations with $\sigma=0.1$, which gives us $\sigma/\mu\approx 100,000\%$. Moreover, in the optimal case, every instance of ESN was shown to implement the required logic perfectly and robustly.
 
 Learning and adaptation is nature's way of working with uncertain structure and reservoir computing gives us a tool to use supervised learning to build computers using uncertain nanoscale self-assembled systems.
 
  The only modification to the structure in RC is to adjust the spectral radius and therefore dynamical regime of the system, which is independent of the implemented logic and can be done using external control signals\cite{doi:10.1162/neco.2007.19.1.111}. Note that in contrast to the RAC model, here we use the controls to adjust the dynamics of the system independently from the tasks. In a physical implementation this adjustment can be performed using body biasing\cite{Wolpert:2012uq}. 
  
  
  
  XXXXX
